Understanding the Effects of the Baidu-ULTR Logging Policy on Two-Tower Models

Despite the popularity of the two-tower model for unbiased learning to rank (ULTR) tasks, recent work suggests that it suffers from a major limitation that could lead to its collapse in industry applications: the problem of logging policy confounding. Several potential solutions have even been proposed; however, the evaluation of these methods was mostly conducted using semi-synthetic simulation experiments. This paper bridges the gap between theory and practice by investigating the confounding problem on the largest real-world dataset, Baidu-ULTR. Our main contributions are threefold: 1) we show that the conditions for the confounding problem are given on Baidu-ULTR, 2) the confounding problem bears no significant effect on the two-tower model, and 3) we point to a potential mismatch between expert annotations, the golden standard in ULTR, and user click behavior.

==> sections/0-abstract.tex <==

\begin{abstract}
    Despite the popularity of the two tower model for unbiased learning to rank (ULTR) tasks, recent work suggest that it suffers from a major limitations that could lead to its collapse in industry applications: the confounding problem. Even a number of potential solutions have been proposed. However, the experiments that these findings are grounded on were conducted on (semi-)synthetic data. The goal of this paper is to bridge the gap between theory and practice by investigating the issue on a real-world dataset. Our main contributions are threefold: 1) we show that the conditions for the confounding problem to arise are met in our dataset, 2) the confounding problem bears no significant effect on the two tower model and 3) we point to a potential mismatch between expert annotations, the golden standard in ULTR, and user click behavior.
\end{abstract}

